Structure-Preserving Reconstruction of Convex Lipschitz Functionals on Hilbert Spaces from Finite Samples

Convex functionals are ubiquitous in applied analysis, appearing as value functions, risk measures, super-hedging prices, and loss functionals in machine learning. In many applications, however, the functional is only observed through finitely many exact pointwise evaluations. We ask whether a convex functional on a separable Hilbert space $H$ can be reconstructed, up to arbitrary uniform accuracy, by an explicit formula which preserves convexity and Lipschitz regularity and is finitely computable. We answer this affirmatively. For every compact convex $C\subseteq H$, every $L$-Lipschitz convex functional $\rho:C\to\mathbb{R}$, and every $\varepsilon>0$, we construct an explicit finite-sample reconstruction which is convex, $L$-Lipschitz, and uniformly $\varepsilon$-accurate on $C$. The construction uses only finitely many linear measurements $\langle b,\cdot\rangle_H$, with $b$ lying in a finite-dimensional subspace of $H$, and is exactly implementable by a $\operatorname{ReLU}$-MLP. Building on this, we introduce convex neural functionals (CNFs), a structured trainable architecture class containing our reconstruction, whose every admissible parameter configuration is automatically convex and Lipschitz, providing a principled foundation for learning convex functionals from finite data.

==> Meetings.tex <==

\begin{enumerate}
    \item \textbf{State:} BSDE Characterization of Time-Consistent Risk-Measures
    \item \textbf{Quote:} 
        Universal Approximation for BSDEs (random-terminal time)
    \item \textbf{Prove/Compute:} 
    Fix $T>0$, If $\tau$ is the first exit time of $X_{\cdot}:=\sigma W_{\cdot}$ where $W_{\cdot}$ is a $2\le d$ Brownian motion from $\bar{B}_2(0,r)$; then for any given error $\varepsilon>0$ and probability of failure $0<\delta \le 1$ how to choose $\sigma,r>0$ such that 
    \begin{equation}
    \label{eq:terminal_time_perturbation}
            \mathbb{P}\big(|\tau-T|<\varepsilon\big)\ge 1-\delta
    .
    \end{equation}
    \item \textbf{Elliptification Lemma - Giulia and Pere?:} \textit{Not sure if this holds under randomization...but I don't se why not}
        If $(Y_{\cdot}^s,Z_{\cdot}^s)$ is ``the same'' BSDE with terminal time $s\in \{t,T\}$ satisfying~\eqref{eq:terminal_time_perturbation} and 
    \[
        \mathbb{P}\Big( \max_{0\le t\le \min\{\tau,T\}}\,
            |Y_{t}^{\tau}-Y_{t}^{T}|
            \in O(\varepsilon)
        \Big)
        \ge 1-\delta
    \]
    (same for $Z_{\cdot}$ simultaneously).
    \item \textbf{To Prove:}
    Use (2) +(4) to deduce approximation of parabolic form of the problem ($T$ not $\tau$).
    \hfill\\
    Deduce good rates in ``nice dynamics'' case.
    \item \textbf{To Prove: Generalization Bounds (Finite Sample Results)} (Maybe):
\end{enumerate}


\subsection{Summary of Feb 25th Meeting}
\begin{enumerate}
    \item BSDEs with random terminal time are more natural for most sources of risk, but terminal time induced by auxiliary forward process' first exit may be questionable
    \item Shift to preliminary problem: approximate (or learn) stopping times (predictable on honest)
    \item \textbf{Questions:}
    \begin{enumerate}
        \item[(i)] What sense do we approximate?  Some options we discussed:change of getting on/off correct - distributional, time itself, distance to correct stopping region, stopping region - as a set?
        \begin{enumerate}
            \item If stochastics: Do we consider $L^p$, $H^p$, or some distributional sense; e.g. $W_p$ or $AW_p$?
        \end{enumerate}
        \item[(ii)] How do approximated stopping times impact BSDEs with random terminal times (can we control approximation/learning error).
    \end{enumerate}
\end{enumerate}
